Geometric Graph Neural Network Modeling of Human Interactions in Crowded Environments

Modeling human trajectories in crowded environments is challenging due to the complex nature of pedestrian behavior and interactions. This paper proposes a geometric graph neural network (GNN) architecture that integrates domain knowledge from psychological studies to model pedestrian interactions and predict future trajectories. Unlike prior studies using complete graphs, we define interaction neighborhoods using pedestrians' field of view, motion direction, and distance-based kernel functions to construct graph representations of crowds. Evaluations across multiple datasets demonstrate improved prediction accuracy through reduced average and final displacement error metrics. Our findings underscore the importance of integrating domain knowledge with data-driven approaches for effective modeling of human interactions in crowds.

==> references <==
\begin{thebibliography}{21}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi:\discretionary{}{}{}#1}\else
  \providecommand{\doi}{doi:\discretionary{}{}{}\begingroup \urlstyle{rm}\Url}\fi

\bibitem[{Alahi et~al.(2016)Alahi, Goel, Ramanathan, Robicquet, Fei-Fei, and Savarese}]{alahi2016social}
Alahi, A., Goel, K., Ramanathan, V., Robicquet, A., Fei-Fei, L., and Savarese, S. (2016).
\newblock Social lstm: Human trajectory prediction in crowded spaces.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, 961--971.

\bibitem[{Grasso et~al.(1998)Grasso, Pr{\'e}vost, Ivanenko, and Berthoz}]{grasso1998eye}
Grasso, R., Pr{\'e}vost, P., Ivanenko, Y.P., and Berthoz, A. (1998).
\newblock Eye-head coordination for the steering of locomotion in humans: an anticipatory synergy.
\newblock \emph{Neuroscience Letters}, 253(2), 115--118.

\bibitem[{Gupta et~al.(2018)Gupta, Johnson, Fei-Fei, Savarese, and Alahi}]{gupta2018social}
Gupta, A., Johnson, J., Fei-Fei, L., Savarese, S., and Alahi, A. (2018).
\newblock Social gan: Socially acceptable trajectories with generative adversarial networks.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, 2255--2264.

\bibitem[{Helbing and Molnar(1995)}]{helbing1995social}
Helbing, D. and Molnar, P. (1995).
\newblock Social force model for pedestrian dynamics.
\newblock \emph{Physical review E}, 51(5), 4282.

\bibitem[{Huang et~al.(2019)Huang, Bi, Li, Mao, and Wang}]{huang2019stgat}
Huang, Y., Bi, H., Li, Z., Mao, T., and Wang, Z. (2019).
\newblock Stgat: Modeling spatial-temporal interactions for human trajectory prediction.
\newblock In \emph{Proceedings of the IEEE/CVF international conference on computer vision}, 6272--6281.

\bibitem[{Kipf and Welling(2016)}]{kipf2016semi}
Kipf, T.N. and Welling, M. (2016).
\newblock Semi-supervised classification with graph convolutional networks.
\newblock \emph{arXiv preprint arXiv:1609.02907}.

\bibitem[{Korbmacher and Tordeux(2022)}]{korbmacher2022review}
Korbmacher, R. and Tordeux, A. (2022).
\newblock Review of pedestrian trajectory prediction methods: Comparing deep learning and knowledge-based approaches.
\newblock \emph{IEEE Transactions on Intelligent Transportation Systems}.

\bibitem[{Kosaraju et~al.(2019)Kosaraju, Sadeghian, Mart{\'\i}n-Mart{\'\i}n, Reid, Rezatofighi, and Savarese}]{kosaraju2019social}
Kosaraju, V., Sadeghian, A., Mart{\'\i}n-Mart{\'\i}n, R., Reid, I., Rezatofighi, H., and Savarese, S. (2019).
\newblock Social-bigat: Multimodal trajectory forecasting using bicycle-gan and graph attention networks.
\newblock \emph{Advances in Neural Information Processing Systems}, 32.

\bibitem[{Lerner et~al.(2007)Lerner, Chrysanthou, and Lischinski}]{lerner2007crowds}
Lerner, A., Chrysanthou, Y., and Lischinski, D. (2007).
\newblock Crowds by example.
\newblock In \emph{Computer graphics forum}, volume~26, 655--664. Wiley Online Library.

\bibitem[{Lv et~al.(2023)Lv, Wang, Wang, Zhang, Xu, and Xu}]{lv2023ssagcn}
Lv, P., Wang, W., Wang, Y., Zhang, Y., Xu, M., and Xu, C. (2023).
\newblock Ssagcn: social soft attention graph convolution network for pedestrian trajectory prediction.
\newblock \emph{IEEE transactions on neural networks and learning systems}.

\bibitem[{Mavrogiannis et~al.(2023)Mavrogiannis, Baldini, Wang, Zhao, Trautman, Steinfeld, and Oh}]{mavrogiannis2023core}
Mavrogiannis, C., Baldini, F., Wang, A., Zhao, D., Trautman, P., Steinfeld, A., and Oh, J. (2023).
\newblock Core challenges of social robot navigation: A survey.
\newblock \emph{ACM Transactions on Human-Robot Interaction}, 12(3), 1--39.

\bibitem[{Mesbahi and Egerstedt(2010)}]{mesbahi2010graph}
Mesbahi, M. and Egerstedt, M. (2010).
\newblock \emph{Graph theoretic methods in multiagent networks}.
\newblock Princeton University Press.

\bibitem[{Mohamed et~al.(2020)Mohamed, Qian, Elhoseiny, and Claudel}]{mohamed2020social}
Mohamed, A., Qian, K., Elhoseiny, M., and Claudel, C. (2020).
\newblock Social-stgcnn: A social spatio-temporal graph convolutional neural network for human trajectory prediction.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 14424--14432.

\bibitem[{Pellegrini et~al.(2009)Pellegrini, Ess, Schindler, and Van~Gool}]{pellegrini2009you}
Pellegrini, S., Ess, A., Schindler, K., and Van~Gool, L. (2009).
\newblock You'll never walk alone: Modeling social behavior for multi-target tracking.
\newblock In \emph{2009 IEEE 12th international conference on computer vision}, 261--268. IEEE.

\bibitem[{Rio et~al.(2018)Rio, Dachner, and Warren}]{rio2018local}
Rio, K.W., Dachner, G.C., and Warren, W.H. (2018).
\newblock Local interactions underlying collective motion in human crowds.
\newblock \emph{Proceedings of the Royal Society B: Biological Sciences}, 285(1878), 20180611.

\bibitem[{Rudenko et~al.(2020)Rudenko, Palmieri, Herman, Kitani, Gavrila, and Arras}]{rudenko2020human}
Rudenko, A., Palmieri, L., Herman, M., Kitani, K.M., Gavrila, D.M., and Arras, K.O. (2020).
\newblock Human motion trajectory prediction: A survey.
\newblock \emph{The International Journal of Robotics Research}, 39(8), 895--935.

\bibitem[{Van Den~Berg et~al.(2011)Van Den~Berg, Guy, Lin, and Manocha}]{van2011reciprocal}
Van Den~Berg, J., Guy, S.J., Lin, M., and Manocha, D. (2011).
\newblock Reciprocal n-body collision avoidance.
\newblock In \emph{Robotics Research: The 14th International Symposium ISRR}, 3--19. Springer.

\bibitem[{Wirth et~al.(2022)Wirth, Dachner, Rio, and Warren}]{wirth2022neighborhood}
Wirth, T.D., Dachner, G.C., Rio, K.W., and Warren, W.H. (2022).
\newblock The neighborhood of interaction in human crowds is neither metric nor topological, but visual.
\newblock \emph{bioRxiv}, 2022--08.

\bibitem[{Yan et~al.(2018)Yan, Xiong, and Lin}]{yan2018spatial}
Yan, S., Xiong, Y., and Lin, D. (2018).
\newblock Spatial temporal graph convolutional networks for skeleton-based action recognition.
\newblock In \emph{Proceedings of the AAAI conference on artificial intelligence}, volume~32.

\bibitem[{Yang et~al.(2023)Yang, Pang, and Zeng}]{yang2023trajectory}
Yang, Z., Pang, C., and Zeng, X. (2023).
\newblock Trajectory forecasting using graph convolutional neural networks based on prior awareness and information fusion.
\newblock \emph{ISPRS International Journal of Geo-Information}, 12(2), 77.

\bibitem[{Zhu et~al.(2021)Zhu, Xu, Zhang, Du, Zhang, Liu, Yang, and Wu}]{zhu2021survey}
Zhu, Y., Xu, W., Zhang, J., Du, Y., Zhang, J., Liu, Q., Yang, C., and Wu, S. (2021).
\newblock A survey on graph structure learning: Progress and opportunities.
\newblock \emph{arXiv preprint arXiv:2103.03036}.

\end{thebibliography}

